Krait: A Backdoor Attack Against Graph Prompt Tuning

Graph prompt tuning has emerged as a promising paradigm to effectively transfer general graph knowledge from pre-trained models to various downstream tasks, particularly in few-shot contexts. However, its susceptibility to backdoor attacks, where adversaries insert triggers to manipulate outcomes, raises a critical concern. We conduct the first study to investigate such vulnerability, revealing that backdoors can disguise benign graph prompts, thus evading detection. We introduce Krait, a novel graph prompt backdoor. Specifically, we propose a simple yet effective model-agnostic metric called label non-uniformity homophily to select poisoned candidates, significantly reducing computational complexity. To accommodate diverse attack scenarios and advanced attack types, we design three customizable trigger generation methods to craft prompts as triggers. We propose a novel centroid similarity-based loss function to optimize prompt tuning for attack effectiveness and stealthiness. Experiments on four real-world graphs demonstrate that Krait can efficiently embed triggers to merely 0.15% to 2% of training nodes, achieving high attack success rates without sacrificing clean accuracy. Notably, in one-to-one and all-to-one attacks, Krait can achieve 100% attack success rates by poisoning as few as 2 and 22 nodes, respectively. Our experiments further show that Krait remains potent across different transfer cases, attack types, and graph neural network backbones. Additionally, Krait can be successfully extended to the black-box setting, posing more severe threats. Finally, we analyze why Krait can evade both classical and state-of-the-art defenses, and provide practical insights for detecting and mitigating this class of attacks.

==> Experiments-ori.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Validation}
\label{sec:exp}
In this section, we conduct empirical experiments based on different types of attacks and trigger generation methods to investigate the following key research questions:

\noindent\textbf{RQ1}: How effective/stealthy is Krait for graph backdoors?

\noindent\textbf{RQ2}: How does Krait perform under diverse combinations of attack types and trigger generation methods? Can it flexibly adapt to different GNN backbones?

\noindent\textbf{RQ3}: What factors can affect the performance of Krait?

\noindent\textbf{RQ4}: Can Krait be extended to the black-box setting?

\subsection{Setups}

\noindent\textbf{Datasets.}
We utilize the same datasets described in Section \ref{sec:prelim_exp}.

\noindent\textbf{Model.}
We set All-in-One \cite{all_in_one} as the victim graph prompt tuning model, using the Graph Transformer (GT) \cite{graph_transformer} as the GNN backbone and GraphCL \cite{graphcl} for pre-training. We consider the multi-class classification setting.

\noindent\textbf{Baselines.}
To the best of our knowledge, Krait is the first graph prompt backdoor, there is no existing method to compare. Therefore, we use random selection and LNH selection respectively to choose poisoned candidates for each type of attack under diverse trigger generation methods as our baselines.

\noindent\textbf{Implementations.}
We follow the default parameter settings in All-in-One \cite{all_in_one}, please refer to more implementation details in Appendix \ref{imp_details}. Besides, we set adaptation steps as $10$, and the trigger size is the same as the graph prompt size, which is $10$. We utilize all nodes in each graph dataset instead of sampling a specific number of nodes for training and testing. We $1$:$1$ split the testing samples, half are clean samples and the rest are attached with triggers. And the coefficient $\alpha=10$. Notably, poisoning rates denote the size of poisoned samples over the size of the target label in the training graph, which is much smaller than the whole size of the training graph or victim graph \cite{unnoticeable_graph_backdoor, data_free_inject}. Since our attack target is mostly the label with the least nodes, the poisoning rates further decrease compared to the existing standards. We report the average results of $5$ trials. All experiments are conducted on a $64$-bit machine with $4$ Nvidia A$100$ GPUs. 

\noindent\textbf{Metrics.}
For benign models, we use accuracy (ACC), F1 score, and AUC to evaluate the performance of node classification. For graph backdoors, to evaluate attack effectiveness, we employ 1) Attack Success Rate (ASR) to quantify how many trigger-injected samples are misclassified to the target label; 2) average misclassification confidence (AMC) \cite{graph_backdoor} to compute the average confidence score assigned to the target label for the successful graph backdoors. To evaluate attack stealthiness, we use 3) poisoning rate (PR) to represent attack budgets; 4) clean accuracy (CA) to measure the classification accuracy of clean samples after backdoor training; 5) average degree difference (ADD) \cite{graph_backdoor} and 6) average homophily difference (AHD) to gauge the degree and local-subgraph homophily differences between clean samples and trigger-injected samples.

\subsection{Attack Performance}
The performance of benign graph prompt tuning is shown in Table \ref{benign_perf}. We observe that transfers from different domains are more unstable, and generally lead to worse performance than within-domain transfers, which fits our intuition. Since there exists at most $4\times4\times3\times3$ cases, based on Table \ref{benign_perf}, we solely pick up $3$ representative cases, namely, CiteSeer to Cora (within-domain, positive, small-to-small transfer), Physics to Computers (out-of-domain, relatively negative, and big-to-big transfer) and Physics to CiteSeer (out-of-domain, positive, and big-to-small transfer) to conduct corresponding experiments. The final performance is presented in Table \ref{Krait_perf}. 
%=====================
% \section{Experimental Validation}
% \label{sec:exp}
% In this section, we conduct empirical experiments based on different types of attacks and trigger generation methods to investigate the following key research questions:

% \textbf{RQ1}: How effective/stealthy is Krait to launch graph backdoors? \par
% \textbf{RQ2}: How Krait perform under diverse combinations of attack types and trigger generation methods? Can it flexibly adapt to different GNN backbones? \par
% \textbf{RQ3}: What factors can affect the performance of Krait? \par
% \textbf{RQ4}: Can Krait be extended to the black-box setting?
% % under varying cases
% \subsection{Set-ups}

% \paragraph{\textbf{Datasets}} We use the same datasets described in Section \ref{sec:prelim_exp}.


% \paragraph{\textbf{Model}}
% We set All-in-One\cite{all_in_one} as the victim graph prompt tuning model, where we leverage Graph Transformer(GT)\cite{graph_transformer} as the GNN backbone and GraphCL\cite{graphcl} to pre-train original graphs. We employ their multi-class classification setting to generate graph prompts. 
% %, instead of transforming node classification tasks into a multi-label problem by training many binary classifiers.

% \paragraph{\textbf{Baselines}}
% To the best of our knowledge, Krait is the first graph prompt backdoor, there is no existing method to compare. Therefore, we treat the random selection and LNH selection strategies respectively to choose poisoned candidates for each type of attack under diverse trigger generation methods as our baselines.
% %, and the random selection strategy with the centroid similarity constraint  against graph prompt tuning

% \paragraph{\textbf{Implementations}} We follow the default parameter settings in All-in-One \cite{all_in_one}, besides, we set adaptation steps as $10$, and the trigger size is the same as the graph prompt size, which is $10$. We $1$:$1$ split the testing samples, half are clean samples and the rest are attached with triggers. And the coefficient $\alpha=10$. Notably, poisoning rates denote the size of poisoned samples over the size of the target label in the training graph, which is much smaller than the whole size of the training graph or victim graph\cite{unnoticeable_graph_backdoor, data_free_inject}. Since our attack target is mostly the label with the least nodes, the poisoning rates further decrease compared to the existing standards. We report the average results of $5$ trials. All experiments are conducted on a $64$-bit machine with $4$ Nvidia A$100$ GPUs. 

% \paragraph{\textbf{Metrics}} For benign models, we leverage $3$ classical metrics, accuracy(ACC), F1, and AUC to evaluate the performance of node classification. For graph backdoors, to evaluate attack effectiveness, we employ 1) ASR to quantify how many trigger-injected samples are misclassified to the target label; 2) average misclassification confidence(AMC)\cite{graph_backdoor}, which denotes the average confidence score assigned to the target label for the successful graph backdoors; to evaluate attack stealthiness, we use 3) poisoning rate(PR) to represent attack budgets, 4) clean accuracy(CA) to quantify the classification accuracy of clean samples after backdoor training; 5) average degree difference(ADD)\cite{graph_backdoor} and 6) average homophily difference(AHD) to measure the degree and local-subgraph homophily difference between clean samples and trigger-injected samples.

% % Trigger-size, test from 1, no larger than graph prompt size.

% % Poisoned samples, at least 10.

% \subsection{Attack Performance}
% The performance of benign graph prompt tuning is shown in Table \ref{benign_perf}. We observe that transfers from different domains are more unstable, and generally lead to worse performance than within-domain transfers, which fits our intuition. Since there exists at most $4\times4\times3\times3$ cases, based on Table \ref{benign_perf}, we solely pick up $3$ representative cases, namely, CiteSeer to Cora(within-domain, positive, small-to-small transfer), Physics to Computers(out-of-domain, relatively negative, and big-to-big transfer) and Physics to CiteSeer(out-of-domain, positive, and big-to-small transfer) to conduct corresponding experiments. The final performance is presented in Table \ref{Krait_perf}. 

%==================

\begin{table}[H]
% \vspace{-2mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc|ccc|ccc|ccc}
\toprule
\textbf{Src\textbackslash{}Tar}  & \multicolumn{3}{c|}{\textbf{Cora}} & \multicolumn{3}{c|}{\textbf{CiteSeer}} & \multicolumn{3}{c|}{\textbf{Physics}} & \multicolumn{3}{c}{\textbf{Computers}} \\ \hline
(Metrics) & ACC     & F1      & AUC   & ACC      & F1      & AUC      & ACC      & F1      & AUC     & ACC      & F1      & AUC      \\ \hline
\textbf{Cora}      & 82.22   & 73.97  & 95.98 & 80.76        & 73.99        & \textbf{91.77}         & \textbf{87.58}         & \textbf{82.51}        & \textbf{94.20}        & 56.46         & 25.62        & 66.18         \\
\textbf{CiteSeer}  & \textbf{86.85}   & \textbf{84.96}   & \textbf{96.63} & \textbf{83.07}        & \textbf{82.37}        & 89.12         & 82.70         & 64.67        & 85.91       & 50.02         & 17.48        & 62.22         \\
\textbf{Physics}   & 72.04  & 59.68 & 88.85 & 80.32        & 77.46        & 91.54         & 79.94         & 67.11        & 87.59        & \textbf{61.92}         & \textbf{28.34}        & \textbf{72.66}         \\
\textbf{Computers} & 47.10  & 25.25 & 67.63   & 54.50       & 40.01        & 78.63         & 79.73         & 59.26       & 81.14       &47.44         & 17.64        & 60.79         \\ \bottomrule
\end{tabular}}
% \captionsetup{justification=raggedright,singlelinecheck=false}
\caption{Performance of benign graph prompt tuning. The row/column denotes the source/target domains, respectively. We bold the best performance in each transfer case.}
\label{benign_perf}
\vspace{-6mm}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{c|c|c|ccccc|ccccc|ccccc}
\toprule
\textbf{Transfer}                      & \multirow{3}{*}{\textbf{Method}}   & \multirow{3}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{One-to-One}}                                                            & \multicolumn{5}{c|}{\textbf{All-to-One}}                                                           & \multicolumn{5}{c}{\textbf{All-to-All}}                                                            \\ \cline{1-1} \cline{4-18} 
(Evaluation)                       &                           &                        & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}}       & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}}      & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c}{\textbf{stealthiness}}       \\ \cline{1-1} \cline{4-18} 
(Metrics)                          &                           &                        & ASR(\%)            & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)            & ASR(\%)             & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)           & ASR(\%)             & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)           \\ \hline
\multirow{9}{*}{\textbf{Cite2Cora}}     & \multirow{3}{*}{\textbf{Invoke}}   & \textbf{Random}                 & 94.22               & 93.12                         & 86.89              & -17.63              & \textbf{0.18}              & 29.10               & 91.49                         & 85.74              & -17.56               & 4.97             & 4.23               & 78.19                         & 85.95              & -17.56               & 9.54             \\
                                   &                           & \textbf{LNH}                    & 95.56               & 93.20                         & \textbf{86.95}              & -17.63               & 0.19              & 38.68               & 90.97                         & 85.39              & -17.56               & 5.02             & 4.05               & 77.95                         & 85.63              & -17.56               & \textbf{9.53}             \\
                                   &                           & \textbf{Full}                  & \textbf{100.00}               & \textbf{100.00}                         & 86.75              & -17.63               & 3.02              & \textbf{100.00}               & \textbf{100.00}                       & \textbf{85.83}              & \textbf{-17.54}               & \textbf{3.24}             & \textbf{6.67}               & \textbf{82.60}                         & \textbf{86.10}              & -17.56               & 10.43             \\ \cline{2-3}
                                       & \multirow{3}{*}{\textbf{Interact}} & \textbf{Random}                 & 42.22 & 86.68           & 86.89 & -17.63 & 0.91 & 99.91 & 99.75            & 85.66 & -17.56 & \textbf{3.65} & \textbf{42.44}  & \textbf{93.96}            & 85.74 & -17.56 & 6.19 \\
                                   &                           & \textbf{LNH}                    & 56.00 & 89.37           & \textbf{86.95} & -17.63 & \textbf{0.82} & 95.51  & 98.86            & 85.68 & -17.56 & 3.71 & 38.38               & 90.53                         & 85.83              & -17.56               & 6.19             \\
                                   &                           & \textbf{Full}                  & \textbf{62.22}               & \textbf{91.77}                         & 86.72              & -17.63               & 1.29              & \textbf{100.00}               & \textbf{100.00}                         & \textbf{85.86}              & -17.56               & 4.05             & 31.78               & 89.51                         & \textbf{86.13}              & -17.56               & \textbf{5.86}             \\ \cline{2-3}
                                   & \multirow{3}{*}{\textbf{Modify}}   & \textbf{Random}                 & 43.56               & 85.88                         & 86.90              & -17.63               & \textbf{0.88}              & \textbf{100.00}               & 99.84                         & 85.66              & -17.56               & \textbf{3.60}             & \textbf{42.61}               & \textbf{93.30}                         & 85.83              & -17.56               & 6.38             \\
                                   &                           & \textbf{LNH}                    & 54.67               & 89.64                         & \textbf{86.98}              & -17.63               & 0.93              & 96.53               & 98.83                         & 85.74              & -17.56               & 3.79             & 38.68               & 89.56                         & 85.83              & -17.56               & 6.13             \\
                                   &                           & \textbf{Full}                  & \textbf{59.56}               & \textbf{91.83}                         & 86.69              & -17.63               & 1.29              & \textbf{100.00}               & \textbf{100.00}                         & \textbf{85.95}              & -17.56               & 4.07             & 31.89               & 89.05                         & \textbf{86.27}              & -17.56               & \textbf{5.80}            \\ \hline
\multirow{9}{*}{\textbf{Phy2Cite}}  & \multirow{3}{*}{\textbf{Invoke}}   & \textbf{Random}                 & 83.64               & 98.76                         & 81.56              & -16.42               & \textbf{9.61}              & 17.14               & 95.05                         & \textbf{81.47}              & -17.93               & \textbf{3.13}             & 8.60                           & \textbf{94.66}              & \textbf{81.11}               & \textbf{-17.90}                  & 3.13        \\
                                   &                           & \textbf{LNH}                    & 78.79               & 97.51                         & 81.78              & -16.42               & 9.64              & 17.89               & 96.40                         & 80.63              & -17.93               & 3.15             & 8.46               & 93.19                         & 79.62              & \textbf{-17.90}               & 3.31             \\
                                   &                           & \textbf{Full}                  & \textbf{100.00}               & \textbf{100.00}                         & \textbf{82.03}              & \textbf{-16.38}               & 11.01              & \textbf{100.00}               & \textbf{100.00}                         & 79.90              & \textbf{-17.88}               & 3.97             & \textbf{8.81}               & 92.17                         & 80.34              & -17.92               & \textbf{2.65}             \\ \cline{2-3}
                                   & \multirow{3}{*}{\textbf{Interact}} & \textbf{Random}                 & 23.64               & 65.49                         & 81.53              & -16.42               & \textbf{9.74}              & 97.98               & 99.81                         & 81.15              & -17.92              & \textbf{3.29}             & 15.87               & 94.00                         & 80.87              & -17.92               & 3.22             \\
                                   &                           & \textbf{LNH}                    & 28.79               & 89.50                         & 80.93              & -16.42               & 10.03              & 82.79               & 98.47                         & 80.00              & -17.92               & 3.39             & 14.45               & 93.84                         & \textbf{80.91}              & -17.92               & \textbf{3.13}             \\
                                   &                           & \textbf{Full}                  & \textbf{31.82}               & \textbf{93.12}                         & \textbf{81.84}              & -16.42               & 10.09              & \textbf{99.93}               & \textbf{100.00}                         & \textbf{81.27}              & -17.92               & 4.02             & \textbf{17.29}               & \textbf{95.58}                         & 79.50              & -17.92               & \textbf{3.13}             \\ \cline{2-3}
                                   & \multirow{3}{*}{\textbf{Modify}}   & \textbf{Random}                 & 21.21               & 89.74                         & \textbf{81.45}              & -16.42               & \textbf{9.70}              & 97.67               & 99.85                         & \textbf{81.30}              & -17.93               & \textbf{3.35}             & 14.17               & 95.01                         & \textbf{81.01}              & -17.92               & 3.24             \\
                                   &                           & \textbf{LNH}                    & 32.42               & 89.45                         & 80.80              & -16.42               & 9.99              & 83.12               & 98.45                         & 80.02              & \textbf{-17.92}              & 3.41             & 15.80               & 94.54                         & 80.36              & -17.92               & 3.51             \\
                                   &                           & \textbf{Full}                  & \textbf{43.33}               & \textbf{92.28}                         & 81.21              & -16.42               & 10.02              & \textbf{99.98}               & \textbf{100.00}                        & 81.03              & \textbf{-17.92}               & 4.01             & \textbf{16.11}               & \textbf{96.25}                         & 79.66              & -17.92               & \textbf{3.04}             \\ \hline
\multirow{9}{*}{\textbf{Phy2Comp}} & \multirow{3}{*}{\textbf{Invoke}}   & \textbf{Random}                 & 53.51               & 95.54                         & 62.21              & -22.94               & -5.19              & 74.42               & 98.00                         & \textbf{62.93}              & -18.75               & \textbf{3.08}             & 4.88               & 93.17                         & 61.02              & -14.81               & 3.10             \\
                                   &                           & \textbf{LNH}                    & 43.24               & 94.62                         & 62.25              & -22.96               & \textbf{-5.30}              & 73.56               & 98.30                         & 60.88              & -18.75               & 3.12             & 3.94               & 93.97                         & 61.67              & -14.97               & \textbf{3.02}             \\
                                   &                           & \textbf{Full}                  & \textbf{99.46}               & \textbf{100.00}                         & \textbf{63.31}              & \textbf{-18.38}               & 4.73             & \textbf{100.00}               & \textbf{100.00}                         & 62.74              & \textbf{-8.31}               & 3.64             & \textbf{25.30}               & \textbf{98.31}                         & \textbf{62.70}              & \textbf{-13.60}               & 3.54             \\ \cline{2-3}
                                   & \multirow{3}{*}{\textbf{Interact}} & \textbf{Random}                 & 25.41               & \textbf{93.02}                         & 60.85              & -23.26               & -5.25              & 98.16               & 99.77                         & 61.20              & -14.34               & \textbf{3.55}             & 5.67               & 95.16                         & 61.50              & -15.93               & 2.97            \\
                                   &                           & \textbf{LNH}                    & 24.05               & 91.85                         & \textbf{62.16}              & -23.36               & \textbf{-5.27}              & 98.14               & 99.78                         & 60.28              & -14.48               & 3.56             & 7.52               & 93.37                         & 61.62              & -16.10               & \textbf{2.73}             \\
                                   &                           & \textbf{Full}                  & \textbf{31.08}               & 91.61                         & 61.70              & \textbf{-23.07}               & -5.19              & \textbf{99.82}               & \textbf{100.00}                         & \textbf{63.75}              & \textbf{-11.76}               & 3.90             & \textbf{18.37}               & \textbf{99.06}                         & \textbf{62.64}             & \textbf{-14.92}              & 3.11             \\ \cline{2-3}
                                   & \multirow{3}{*}{\textbf{Modify}}   & \textbf{Random}                 & 34.86               & \textbf{94.35}                         & 62.15              & -23.32               & -5.23              & 98.76               & 99.84                         & 60.19              & -14.67               & \textbf{3.51}             & 6.13               & 96.51                         & 61.17              & -15.83               & 3.15             \\
                                   &                           & \textbf{LNH}                    & 26.49               & 92.26                         & \textbf{62.28}              & -23.21               & \textbf{-5.28}              & 98.26               & 99.79                         & 60.01              & -13.96               & \textbf{3.51}             & 10.50               & 95.72                      & \textbf{61.76}              & -16.68               & \textbf{2.55}             \\
                                   &                           & \textbf{Full}                  & \textbf{38.11}               & 90.45                         & 61.69              & \textbf{-23.12}               & -5.20              & \textbf{99.56}               & \textbf{99.98}                         & \textbf{62.89}              & \textbf{-11.73}               & 3.94             & \textbf{17.75}               & \textbf{98.95}                         & 59.87              & \textbf{-14.37}               & 3.16             \\ \hline
\end{tabular}
}
% \captionsetup{justification=raggedright,singlelinecheck=false}
\caption{Performance of Krait under the white-box setting. Cite2Cora: CiteSeer to Cora transfer; Phy2Cite: Physics to CiteSeer transfer; Phy2Comp: Physics to Computers transfer. Random and LNH denote poison node selection strategies, and Full denotes Krait. We bold the best performance under different combinations of attack types and trigger generation methods.}
\label{Krait_perf}
% \vspace{-5mm}
\end{table*}
To address RQ1 and RQ2, we compare Krait with baselines under various attack types and trigger generation methods across three transfer cases.

\noindent\textbf{Effectiveness.}
% According to the results shown in Table \ref{Krait_perf}, Krait consistently outperforms the baselines in terms of Attack Success Rate (ASR) and Average Misclassification Confidence (AMC), particularly in big-to-big and big-to-small transfers. In almost all scenarios, Krait achieves higher attack effectiveness compared to the baselines. Notably, employing a label non-uniformity homophily strategy without constraints serves as an ablation study, where most attacks either surpass or match the performance of random triggers.
As shown in Table \ref{Krait_perf}, we observe that Krait consistently outperforms the baselines in terms of ASR and AMC, particularly in big-to-big and big-to-small transfers. In almost all attacks, Krait accomplishes higher attack effectiveness compared to the baselines. Notably, solely employing a label non-uniformity homophily strategy without constraints serves as an ablation study, where Krait surpasses or achieves considerable attack performances than random triggers in the most of attack pairs. 

\noindent\textbf{Stealthiness.}
% For a fair comparison, we standardize the poisoning rate (PR) at 2\% for all experiments, with the overall PR relative to the entire training graph ranging between 0.15\% and 2\% for the three attack types, significantly lower than the typical standards of 5\% and 10\%. In one-to-one attacks involving small-scale transfers, poisoned samples include only two nodes, yet in more complex scenarios, Krait poisons about 20 nodes but typically achieves 100\% ASR. Moreover, compared to the classification accuracy of all test samples reported in Table \ref{benign_perf}, all attacks maintain or even improve clean accuracy, demonstrating Krait's stealthiness. Statistically, Krait increases node degrees in poisoned samples, a discrepancy that can be obscured by graph prompt tuning's tendency to significantly expand average node degrees and thereby diminish overall homophily. Additionally, Krait effectively evades detection by homophily and node similarity-based defenses\cite{unnoticeability_node_centric_homo}, as it generally preserves the homophily characteristics inherent in graph prompt tuning and integrates triggers based on node similarity between the triggers and clean (prompted) graphs.
For a fair comparison, we set the PR as $2$\% for all experiments, with the overall PR relative to the entire training graph ranging between $0.15$\% and $2$\% for the three attack types, which is significantly lower than the typical standard of $10\%$ in graph backdoor attacks. In one-to-one attacks for small-scale transfers, poisoned samples contain only two nodes; even in more complex scenarios, Krait only poisons $22$ nodes but achieves $100$\% ASR. Besides, compared to the benign classification accuracy of all test samples reported in Table \ref{benign_perf}, Krait achieves comparable clean accuracy or even surpasses the benign results in all attack types, demonstrating its stealthiness. Regarding statistical properties, Krait introduces larger node degrees in poisoned samples. However, this discrepancy can be obscured by graph prompt tuning as it attaches an extra subgraph into each ego-network, significantly enlarging average node degrees. Additionally, Krait effectively evades detection against homophily and node similarity-based defenders \cite{unnoticeability_node_centric_homo}, since the overall homophily changes between clean samples and poisoned nodes are slight. Moreover, Krait naturally inherits mechanisms of graph prompt tuning to generate graph prompts based on node similarities, whereas it treats prompts as triggers. This characteristic makes Krait more difficult to be detected by node-similarity defenders. We further discuss the details in Subsection \ref{discuss_def}.

\noindent\textbf{Practicability.}
% From the data in Table \ref{Krait_perf}, Krait exhibits outstanding performance with ASRs of 99.56\%-100\% in all-to-one attacks, regardless of the trigger generation method used. The 'Invoke' method performs exceptionally well in one-to-one attacks, achieving ASRs between 99.46\% and 100\%, while the 'Interact' method leads in all-to-all attacks, with ASRs ranging from 6.67\% to 31.89\%. The lower performance in all-to-all attacks is expected as Krait uses a universal trigger, differing from the specific triggers used in backdoors against computer vision (CV) models\cite{first_work,all_to_one_all} that require distinct triggers for each attack pair. In practice, attackers can consider their resources, capabilities, and preferences to select the most suitable trigger generation method.
As shown in Table \ref{Krait_perf}, Krait exhibits superior performance with ASRs of $99.56\%-100\%$ in all-to-one attacks across all trigger generation methods. The ``Invoke" method excels in one-to-one attacks, achieving ASRs between $99.46\%$ and $100\%$, while the ``Interact" method stands out in all-to-all attacks, with ASRs ranging from $6.67\%$ to $31.89\%$. The relatively lower performance in all-to-all attacks is reasonable since Krait employs a universal trigger, differing from the specific triggers used in the computer vision (CV) domain \cite{first_work,all_to_one_all} that require learning distinct triggers for each attack victim and target pair. In real-world applications, attackers can consider their resources, capabilities, preferences, and involved stages to select the most suitable trigger generation method.

% \paragraph{\textbf{Flexibility}} We select $3$ attack type and trigger generation combinations, namely, 'Invoke' for one-to-one attacks, 'Interact' for all-to-one attacks, and 'Modify' for all-to-all attacks to report our results in the CiteSeer to Cora transfer case. Except for GT\cite{graph_transformer}, we additionally employ the graph convolutional network(GCN)\cite{GCN} and graph attention network(GAT)\cite{GAT} as GNN backbones. From Table \ref{backbone_Krait}, we observe that Krait still maintains superior performance in view of attack effectiveness and stealthiness.
\noindent\textbf{Flexibility.}
% We test three combinations of attack types and trigger generation methods—'Invoke' for one-to-one attacks, 'Interact' for all-to-one attacks, and 'Modify' for all-to-all attacks—in the CiteSeer to Cora transfer case. Besides using the Graph Transformer (GT)\cite{graph_transformer}, we also incorporate Graph Convolutional Network (GCN)\cite{GCN} and Graph Attention Network (GAT)\cite{GAT} as alternative GNN backbones. Results in Table \ref{backbone_Krait} indicate that Krait maintains excellent performance in terms of both attack effectiveness and stealthiness across different GNN backbones.
We select three combinations of attack types and trigger generation methods, namely, ``Invoke" for one-to-one attacks, ``Interact" for all-to-one attacks, and ``Modify" for all-to-all attacks to report our results in the CiteSeer to Cora transfer case. Except for GT \cite{graph_transformer}, we additionally employ the graph convolutional network (GCN) \cite{GCN} and graph attention network (GAT) \cite{GAT} as GNN backbones. As shown in Table \ref{backbone_Krait}, Krait maintains superior performance in terms of attack effectiveness and stealthiness across different GNN backbones.
%===========
% To answer RQ$1 \&2$, we compare Krait with baselines under various attack types and trigger generation methods in $3$ transfer cases.

% \paragraph{\textbf{Effectiveness}} From Table \ref{Krait_perf}, we observe that Krait overall outperforms baselines in terms of ASR and AMC, especially in big-to-big and big-to-small transfers, almost all attacks accomplish higher attack effectiveness compared to baselines. Notably, solely choosing a label non-uniformity homophily strategy without constraints can be treated as the ablation study. Most of the attacks exceed or achieve considerable attack performances than random triggers. 


% \paragraph{\textbf{stealthiness}}
% To better compare, we set the PR as $2\%$ for all experiments, and the overall PR respect to the whole training graph is around $[0.15\%, 2\%]$ for $3$ different attack types, which is much lower than current standards, i.e., $5\%,\ 10\%$. In the one-to-one attacks for small-scale transfers, poisoned samples only contain $2$ nodes, even in more advanced attacks, Krait only poisons around $20$ nodes but mostly achieves $100\%$ ASR. Besides, in contrast to the classification accuracy of all test samples shown in Table \ref{benign_perf}, all attacks retain comparable clean accuracy or even surpass the benign results, which proves the stealthiness of Krait. As for statistical properties, compared to clean samples, Krait introduces larger node degrees in the poisoned nodes, however, this situation can be hidden behind graph prompt tuning as it immensely enlarges average node degrees and thus reduces homophily of the whole downstream graphs. Additionally, Krait is evasive to homophily and node similarity-based defenders\cite{unnoticeability_node_centric_homo} since the overall homophily changes are acceptable, and Krait in essence inherits the characteristics of graph prompt tuning, thereby implanting triggers based on the node similarity between triggers and clean (prompted)graphs.

% \paragraph{\textbf{Practicability}} From Table \ref{Krait_perf}, Krait outperforms with $99.56$-$100\%$ ASR for all-to-one attacks regardless of trigger generation methods. Besides, the 'Invoke' method yields better performance with $99.46$-$100\%$ ASR in one-to-one attacks, while the 'Interact' method beats others in all-to-all attacks with $6.67$-$31.89\%$. The relatively degraded performances in all-to-all attacks are reasonable since Krait resorts to a universal trigger to launch attacks, which is distinct from existing backdoors against computer vision(CV) models\cite{first_work,all_to_one_all} that learn separate triggers for any attack pairs. In real practice, attackers can ponder their resources, capabilities, and preferences to choose the corresponding 'optimal' combinations.

% \paragraph{\textbf{Flexibility}} We select $3$ attack type and trigger generation combinations, namely, 'Invoke' for one-to-one attacks, 'Interact' for all-to-one attacks, and 'Modify' for all-to-all attacks to report our results in the CiteSeer to Cora transfer case. Except for GT\cite{graph_transformer}, we additionally employ the graph convolutional network(GCN)\cite{GCN} and graph attention network(GAT)\cite{GAT} as GNN backbones. From Table \ref{backbone_Krait}, we observe that Krait still maintains superior performance in view of attack effectiveness and stealthiness.

%=================
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!htbp]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|ccccc|ccccc|ccccc}
\toprule
\textbf{Transfer}                  & \multirow{3}{*}{\textbf{Backbone}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{One-to-One(Invoke)}}                                                      & \multicolumn{5}{c|}{\textbf{All-to-One(Interact)}}                                                      & \multicolumn{5}{c}{\textbf{All-to-All(Modify)}}                                                      \\ \cline{1-1} \cline{4-18} 
    (Evaluation)                   &                           &                        & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}} & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}} & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c}{\textbf{stealthiness}} \\ \cline{1-1} \cline{4-18} 
(Metrics)                      &                           &                        & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD          & AHD(\%)         & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD          & AHD(\%)         & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD         & AHD(\%)         \\ \hline
\multirow{9}{*}{\textbf{Cite2Cora}} & \multirow{3}{*}{\textbf{GCN}}   & \textbf{Random}                 & 16.00          & 82.91                              & 87.70            & -17.58             & 6.79            & 98.24          & \textbf{99.12}                              & 86.57           & -17.57             & 5.25            & \textbf{31.25}          & 93.77                              & \textbf{86.75}            & -17.57            & 4.58            \\
                               &                           & \textbf{LNH}                    & 30.67          & 84.36                              & \textbf{87.73}            & -17.58             & \textbf{6.62}            & \textbf{98.59}          & 99.10                              & 86.77            & -17.57             & 5.72            & 27.75          & 90.12                              & 86.54            & -17.57            & \textbf{3.94}            \\
                               &                           & \textbf{Full}                  & \textbf{86.89}          & \textbf{95.75}                              & \textbf{87.73}            & \textbf{-15.13}             & 9.94            & 94.13          & 98.70                              & 86.45            & \textbf{-17.47}             & 6.63            & 26.81          & \textbf{94.49}                              & 86.36            & -17.57            & 4.13            \\ \cline{2-3}
                               & \multirow{3}{*}{\textbf{GAT}} & \textbf{Random}                 & 60.44          & 93.32                              & 69.52            & -17.63             & \textbf{0.59}            & 99.38          & 99.97                              & 66.33            & -17.56             &  \textbf{4.94}           & \textbf{16.42}          & 91.15                              & \textbf{68.13}            & -17.56            & 5.06            \\
                               &                           & \textbf{LNH}                    & 66.67          & 94.73                              & 71.67            & -17.63             & 0.63            & 99.21         & 99.95                              & 67.30            & -17.56            & 5.16            & 16.24          & \textbf{93.32}                              & 67.72            & -17.56            & 5.52            \\
                               &                           & \textbf{Full}                  & \textbf{100.00}          & \textbf{99.80}                              & \textbf{71.91}            & \textbf{-17.60}             & 3.34            & \textbf{100.00}          & \textbf{100.00}                              & \textbf{68.57}            & -17.56             & 5.44            & 13.63          & 89.35                              & 66.22            & -17.56            & \textbf{4.96}            \\ \cline{2-3}
                               & \multirow{3}{*}{\textbf{GT}}   & \textbf{Random}                 &94.22               & 93.12                         & 86.89              & -17.63               & \textbf{0.18}             & 99.91 & 99.75            & 85.66 & -17.56 & \textbf{3.65}             & \textbf{42.61}               & \textbf{93.30}                         & 85.83              & -17.56               & 6.38            \\
                               &                           & \textbf{LNH}                    & 95.56               & 93.20                         & \textbf{86.95}              & -17.63               & 0.19             & 95.51  & 98.86           & 85.68 & -17.56 & 3.71             & 38.68               & 89.56                         & 85.83              & -17.56               & 6.13             \\
                               &                           & \textbf{Full}                  & \textbf{100.00}               & \textbf{100.00}                         & 86.75              & -17.63               & 3.02             & \textbf{100.00}               & \textbf{100.00}                         & \textbf{85.86}              & -17.56               & 4.05             & 31.89               & 89.05                         & \textbf{86.27}              & -17.56               & \textbf{5.80}             \\ \bottomrule
\end{tabular}}
% \captionsetup{justification=raggedright,singlelinecheck=false}
\caption{Performance of Krait under different GNN backbones. Cite2Cora: CiteSeer to Cora transfer.}
\label{backbone_Krait}
\vspace{-6mm}
\end{table*}

\subsection{Parameter Studies} To answer RQ$3$, we conduct parameter studies on trigger size, PR, epochs, and constraint coefficient, respectively.

\noindent\textbf{Trigger size.} We vary trigger size as $[1,5,10,15,20]$. As shown in Figure \ref{tri_size}, Krait consistently surpasses the baselines as the trigger size increases. Notably, even with the trigger size set to $1$, Krait can still achieve $100\%$ ASR in one-to-one and all-to-one attacks. However, larger trigger sizes in all-to-all attacks may result in ASR drops. We speculate that since Krait generates a universal trigger for all given attack pairs, it can continuously encode the general malicious knowledge to facilitate graph backdoor attacks before the trigger size reaches an ``optimal" threshold. As trigger size grows, Krait may encode redundant information, leading to ASR drops. Sun et al. \cite{all_in_one} report similar observations when increasing the size of the prompt token.
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\linewidth]{para_tri_size_new.png}
  % \captionsetup{justification=raggedright,singlelinecheck=false}
  \caption{Impact of trigger size in Krait, x-axis denotes the trigger size while y-axis denotes the ASR.}
  \label{tri_size}
  \vspace{-4mm}
\end{figure}

\noindent\textbf{Poisoning rate.} We vary PR as $[2,5,10,20,50]\%$. From Figure \ref{pr}, generally, higher PR, higher ASR. Except for all-to-all attacks, the rest of the attacks with disparate trigger generation methods all accomplish $100\%$ ASR with less than $5\%$ PR. 
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{para_poi_rate.png}
  % \captionsetup{justification=raggedright,singlelinecheck=false}
  \caption{Impact of poisoning rate in Krait, x-axis denotes the PR while y-axis denotes the ASR.}
  \label{pr}
  \vspace{-4mm}
\end{figure}

\noindent\textbf{Training epochs.} We vary training epochs as $[2,4,6,8,10]$. As shown in Figure \ref{train_epoch}, generally, larger epochs yield higher ASRs. In one-to-one attacks with the ``Invoke" method, only training for $2$ epochs with $2$ poisoned nodes yields $100\%$ ASR, and in all-to-one attacks, within $4$ training epochs, Krait achieves $100\%$ ASR with $22$ poisoned nodes.
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{para_epoch.png}
  % \captionsetup{justification=raggedright,singlelinecheck=false}
  \caption{Impact of training epochs in Krait, x-axis denotes the PR while y-axis denotes the ASR.}
  \label{train_epoch}
  \vspace{-4mm}
\end{figure}

\noindent\textbf{Constraint coefficient.}
We vary $\alpha$ as $[0.1, 0.5, 1, 2, 5]$. Interestingly, as shown in Figure \ref{cons_coeff}, these three trigger generation methods perform differently for various attack types. In one-to-one attacks, ``Invoke" stands out with $100\%$ ASR while ``Interact" and ``Modify" behave almost the same, where their ASRs first increase and then decrease. Similar patterns are observed in all-to-one attacks, but they all maintain $100\%$ ASR with $\alpha$ less than $2$. In all-to-one attacks, the ASRs for ``Invoke" monotonically increase, whereas those for ``Interact'' and ``Modify'' both decline.  
\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{para_alpha.png}
  % \captionsetup{justification=raggedright,singlelinecheck=false}
  \vspace{-3mm}
  \caption{Impact of the coefficient alpha in Krait, x-axis denotes the alpha while y-axis denotes the ASR.}
  \label{cons_coeff}
  \vspace{-4mm}
\end{figure}


\subsection{Black-box Setting}
We consider a more practical setting where the system or platform does not support custom training and there is no access to intermediate results. To address this black-box setting, Krait can be degraded into the ``Invoke" trigger generation method without the constraint. We leverage All-in-one with different GNN backbones to mimic the open-sourced models in poisoning warm-ups. We set $\alpha\in$(0.1,0.6). Due to the harsh setting, we set PR as $10\%$, which only poisons $9$ nodes in one-to-one attacks and $96$ nodes in all-to-one attacks ($0.67\%,7\%$ of the whole training graph, respectively), still much lower than the existing standard in graph backdoor attacks. The results are shown in Table \ref{black_Krait}. Under diverse GNN backbones, the black-box Krait still yields comparable performance in terms of attack effectiveness and stealthiness. Krait with the same GT backbone (but with different parameters) achieves superior performance in one-to-one and all-to-one attacks, and Krait with the GCN backbone excels in all-to-all attacks with a $35.95\%$ ASR but it leads to large homophily drops.  
%if the system does not support custom training thus no access to intermediate results, the black-box Krait can be degraded into the 'Invoke' trigger generation methods without the constraint, 
% Consider different classifiers or not???

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!htbp]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|ccccc|ccccc|ccccc}
\hline
\textbf{Transfer}                  & \multirow{3}{*}{\textbf{Backbone}}   & \multirow{3}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{One-to-One}}                                                      & \multicolumn{5}{c|}{\textbf{All-to-One}}                                                      & \multicolumn{5}{c}{\textbf{All-to-All}}                                                      \\ \cline{1-1} \cline{4-18} 
(Evaluation)                   &                           &                        & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}} & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}} & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c}{\textbf{stealthiness}} \\ \cline{1-1} \cline{4-18} 
(Metrics)                      &                           &                        & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD          & AHD(\%)         & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD          & AHD(\%)         & ASR(\%)       & \multicolumn{1}{c|}{AMC(\%)}      & CA(\%)          & ADD         & AHD(\%)         \\ \hline
\multirow{9}{*}{\textbf{Cite2Cora}} & \multirow{3}{*}{\textbf{GCN}}   & \textbf{Random}                 & 34.22          & 78.65                              & \textbf{86.83}            & -17.63             & 9.53           & 32.13          & 93.48                              & \textbf{85.07}            & -17.56            & 9.63            & \textbf{35.95}          & \textbf{95.25}                              & 85.48            & -17.33            & 19.77            \\
                               &                           & \textbf{LNH}                    & \textbf{43.56}          & \textbf{85.39}                              & 86.81            & -17.63             & \textbf{9.41}            & 44.88          & 92.50                              & 84.33            & -17.56             & \textbf{9.36}            & 31.45          & 90.80                              & 86.10            & -17.33            & \textbf{19.65}            \\
                               &                           & \textbf{Full}                  & 41.33          & 70.16                              & 86.81            & \textbf{-15.18}             & 14.59            & \textbf{98.41}          & \textbf{99.07}                             & 84.59            & \textbf{-16.15}             & 11.45            & 30.25          & 91.54                              & \textbf{86.16}            & \textbf{-17.29}            & 19.96            \\ \cline{2-3}
                               & \multirow{3}{*}{\textbf{GAT}} & \textbf{Random}                 & 4.44          & 35.36                             & \textbf{87.10}            & -17.63             & -1.09            & 41.00          & 94.46                              & \textbf{84.92}            & -17.56             & 4.16            & \textbf{13.01}          & \textbf{76.34}                              & 85.60            & -17.56            & 3.40            \\
                               &                           & \textbf{LNH}                    & 8.89         & 45.90                              & 87.04            & -17.63             & \textbf{-1.12}            & 51.07          & 92.82                              & 84.21            & -17.56             & 4.18            & 6.78          & 71.49                              & \textbf{85.83}            & -17.56            & 3.35            \\
                               &                           & \textbf{Full}                  & \textbf{26.67}          & \textbf{67.60}                              & 86.97            & \textbf{-17.56}             & 1.79            & \textbf{71.48}          & \textbf{94.47}                              & 84.33            & \textbf{-17.54}             & \textbf{2.93}            & 6.23          & 70.94                              & 85.71            & -17.56            & \textbf{2.95}            \\ \cline{2-3}
                               & \multirow{3}{*}{\textbf{GT}}   & \textbf{Random}                 & 98.67               & 96.67                         & \textbf{87.00}              & -17.63               & 0.34              & 97.03               & 97.35                         & 82.92              & -17.56               & 4.89             & 7.02               & 78.51                         & \textbf{85.95}              & -17.56               & 9.72             \\
                                   &                           & \textbf{LNH}                    & 97.78               & 95.04                         & 86.90              & -17.63               & \textbf{0.30}              & 90.66               & 95.23                         & 83.12              & -17.56               & 4.91                & 4.43               & 77.81                         & 85.94              & -17.56               & \textbf{9.58}             \\
                                   &                           & \textbf{Full}                  & \textbf{100.00}               & \textbf{100.00}                         & 86.95              & -17.63               & 2.73              & \textbf{100.00}               & \textbf{100.00}                         & \textbf{85.71}              & \textbf{-17.54}               & \textbf{3.08}             & \textbf{8.81}               & \textbf{85.03}                         & 85.66              & -17.56               & 10.32              \\ \hline
\end{tabular}}
% \captionsetup{justification=raggedright,singlelinecheck=false}
\caption{Performance of Krait under the black-box setting. Cite2Cora: CiteSeer to Cora transfer.}
\label{black_Krait}
\vspace{-4mm}
\end{table*}

\subsection{Discussions}
\label{discuss_def}

\noindent\subsubsection{\textbf{Possible Defense Solutions}}
% Given that defense mechanisms against graph backdoor attacks are still in their infancy, we explore strategies from other graph adversarial attacks and injection-based backdoor detections in different domains to assess their effectiveness against Krait.

% \paragraph{\textbf{Homophily and Node-Similarity Defenders.}}
% Authors in \cite{unnoticeability_node_centric_homo} suggest homophily defenders for graph injection attacks, and demonstrate that GNNGuard\cite{gnnguard}, an acclaimed defense mechanism \cite{contrastive_backdoor}, acts as a homophily defender by pruning suspicious edges if 
% $sim(X_v, X_u)\leq s_{\mathcal{G}}$, where $s_{\mathcal{G}}$ denotes the minimum similarity for any pair of nodes connected in $\mathcal{G}$. However, this defense is less effective against Krait for several reasons: 1) As detailed in Section \ref{sec:prelim_exp}, the consistent homophily patterns before and after graph prompt backdoor injections make it challenging for defenders to pinpoint poisoned nodes; 2) Homophily defenders are primarily designed for node classification tasks, but graph prompt tuning models reframe these tasks as graph classification challenges, complicating the detection of small-scale node injections in each ego-network. As evidenced in Tables \ref{Krait_perf}-\ref{black_Krait}, homophily variations between clean and poisoned samples are typically minimal; 3) The structure of prompt tokens, which are similarity functions of token features, can be adaptively tuned when generating poisoned prompts, making them difficult to disrupt by homophily defenders. This challenge also extends to node similarity-based detectors mentioned in \cite{motif_backdoor}.

% As for GNN-Jaccard\cite{gnn_jaccard}, which uses Jaccard similarity to filter out suspicious nodes based on feature overlaps, it is less effective because many graph prompt tuning models\cite{all_in_one} employ dimensionality reduction techniques, particularly in large-scale graphs with nearly 10,000 node features\cite{physics_computers}, thus complicating trigger identification.

% \paragraph{\textbf{Model Inspection.}}
% Adapting strategies like NeuralCleanse\cite{neural_cleanse} for the graph domain involves computing the graph edit distance between triggers and the subgraphs they replace. However, since Krait does not require subgraph replacement and can camouflage triggers as benign prompts within victim ego-networks, it diminishes the effectiveness of such backdoor detection techniques.

% \paragraph{\textbf{Randomized Smoothing.}}
% Randomized smoothing\cite{random_backdoor} is another potential defense approach, which relies on sampling numerous subgraphs of each ego-network to conduct significant majority voting. However, applying this strategy to graph prompt backdoors proves impractical due to the prohibitive computational costs associated with processing multiple subgraphs for each ego-network.

%==========================
% \subsubsection{\textbf{Possible Defense Solutions}}

\begin{table*}[htbp]
\resizebox{\linewidth}{!}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{c|c|c|ccccc|ccccc|ccccc}
\toprule
\textbf{Transfer}                      & \multirow{3}{*}{\textbf{Method}}   & \multirow{3}{*}{\textbf{Model}} & \multicolumn{5}{c|}{\textbf{One-to-One}}                                                            & \multicolumn{5}{c|}{\textbf{All-to-One}}                                                           & \multicolumn{5}{c}{\textbf{All-to-All}}                                                            \\ \cline{1-1} \cline{4-18} 
(Evaluation)                       &                           &                        & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}}       & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c|}{\textbf{stealthiness}}      & \multicolumn{2}{c|}{\textbf{Effectiveness}} & \multicolumn{3}{c}{\textbf{stealthiness}}       \\ \cline{1-1} \cline{4-18} 
(Metrics)                          &                           &                        & ASR(\%)            & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)            & ASR(\%)             & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)           & ASR(\%)             & \multicolumn{1}{c|}{AMC(\%) } & CA(\%)             & ADD            & AHD(\%)           \\ \hline
\multirow{9}{*}{\textbf{Cite2Cora}}     
& \multirow{3}{*}{\textbf{Invoke}}   
                                  & \textbf{GNN-SVD}                 
                                  & 100.00               & 100.00                         & \textbf{86.77}              & -17.62              & \textbf{7.71}              
                                  & 100.00               & 100.00                         & 85.83              & -17.43               & \textbf{6.02}             
                                  & 6.90               & 82.50                         & \textbf{86.13}              & -17.43               & \textbf{15.72}             \\
                                  & 
                                   & \textbf{NoisyGNN-Fea}                    
                                   & 100.00               & 100.00                         & 86.72              & \textbf{-17.63}               & 3.23              
                                   & 100.00               & 100.00                         & \textbf{85.95}              & \textbf{-17.54}              & 3.54             
                                   & \textbf{6.11}               & \textbf{80.71}                         & 86.07              & \textbf{-17.56}               & 10.54   
                                   \\
                                   &                           
                                   & \textbf{NoisyGNN-Emb}                    
                                   & 100.00               & 100.00                         & 86.75              & \textbf{-17.63}               & 3.02              
                                   & 100.00               & 100.00                         & 85.83              & \textbf{-17.54}               & 3.27             
                                   & 6.75               & 81.74                         & 86.07              & \textbf{-17.56}               & 10.44    \\    
                                    \cline{2-3}
& \multirow{3}{*}{\textbf{Interact}} 
                                   & \textbf{GNN-SVD}                 
                                   & \textbf{61.78} & 91.90           & 86.69 & -17.61 & \textbf{7.89} 
                                   & 100.00 & 100.00            & 85.89 & -17.44 & \textbf{7.91} 
                                   & \textbf{31.01}  & \textbf{89.74}            & 86.16 & -17.44 & \textbf{11.29} \\
                                   & 
                                   & \textbf{NoisyGNN-Fea}                    
                                   & 64.44               & \textbf{89.72}                         & 86.65              & \textbf{-17.63}               & 1.60              
                                   & 100.00               & 100.00                         & \textbf{86.13}              & \textbf{-17.56}               & 4.32             
                                   & 31.45               & 90.71                         & 86.16              & \textbf{-17.56}               & 6.07                  
                                   \\
                                   &                           
                                   & \textbf{NoisyGNN-Emb}                    
                                   & 63.56 & 90.65           & \textbf{86.71} & \textbf{-17.63} & 1.29 
                                   & 100.00  & 100.00            & 85.86 & \textbf{-17.56} & 4.05 
                                   & 31.89               & 88.47                         & \textbf{86.22}              & \textbf{-17.56}               & 5.96        \\    
                                    \cline{2-3}
& \multirow{3}{*}{\textbf{Modify}}   
                                   & \textbf{GNN-SVD}                 
                                   & \textbf{60.89}               & 90.20                         & \textbf{86.69}              & \textbf{-17.89}               & \textbf{5.63}              
                                   & 100.00               & 100.00                         & 85.92              & \textbf{-17.65}               & \textbf{6.61}             
                                   & \textbf{31.60}               & \textbf{89.50}                         & \textbf{86.27}              & \textbf{-17.65}               & \textbf{9.83}             \\
                                   & 
                                   & \textbf{NoisyGNN-Fea}                    
                                   & 64.00               & \textbf{88.27}                         & 86.62              & -17.63               & 1.61              
                                   & 100.00               & 100.00                         & \textbf{86.01}              & -17.56               & 4.35             
                                   & 31.78               & 88.99                         & 86.24              & -17.56               & 6.11                    \\
                                   &                           
                                   & \textbf{NoisyGNN-Emb}                    
                                   & 61.78               & 90.53                         & \textbf{86.69}              & -17.63               & 1.29              
                                   & 100.00               & 100.00                         & 85.92              & -17.56               & 4.06             
                                   & 31.81               & 88.61                         & 86.22              & -17.56               & 5.82        \\    
                                    \hline
\end{tabular}
}
% \captionsetup{justification=raggedright,singlelinecheck=false}
\caption{Performance of Krait on GNN-SVD, NoisyGNN-Fea and NoisyGNN-Emb. Cite2Cora: CiteSeer to Cora transfer.}
\label{krait_defense}
\vspace{-6mm}
\end{table*}

Given that defense mechanisms against graph backdoor attacks are still in their infancy, we resort to defenses from other graph adversarial attacks and injection-based backdoor detections in different domains to analyze and assess their effectiveness against Krait.

\noindent\textbf{Homophily and node-similarity defenders.}
Chen et al. \cite{unnoticeability_node_centric_homo} propose homophily defenders against graph injection attacks and demonstrate that GNNGuard \cite{gnnguard}, an acclaimed defense mechanism \cite{contrastive_backdoor}, acts as a homophily defender by pruning suspicious edges if $sim(X_v, X_u)\leq s_{\mathcal{G}}$, where $s_{\mathcal{G}}$ denotes the minimum similarity for any pair of nodes connected in $\mathcal{G}$. Nonetheless, GNNGuard becomes ineffective against Krait for the following four reasons: 1) As indicated in Section \ref{sec:prelim_exp}, the consistent homophily patterns before and after graph prompt backdoor injections make it more intractable for defenders to identify poisoned nodes; 2) GNNGuard is primarily designed for node classification and cannot be trivially applied to graph prompt backdoor attacks since the latter reformulate node-level tasks to graph-level tasks, complicating the detection of small-scale trigger injection in each ego-network. Meanwhile, as shown in Table \ref{Krait_perf}-\ref{black_Krait}, homophily variations between clean samples and poisoned nodes are typically slight; 3) The structure of prompt tokens, which are mainly similarity functions of token features, can be adaptively tuned when crafting poisoned prompts, making them more difficult for homophily defenders to defeat. This challenge likewise extends to node similarity-based detectors mentioned in \cite{motif_backdoor}; 4) Ennadir et al. \cite{NoisyGNN} empirically validate that homophily defenders, i.e., GNNGuard, are $11.78-303.43$ times slower than other defense mechanisms. GNN-Jaccard \cite{gnn_jaccard}, which utilizes Jaccard similarity (only count $0$ or $1$) to remove suspicious edges if their linked nodes' similarity scores are close to $0$, will lose efficacy since the myriad of graph prompt tuning models \cite{all_in_one} employ dimensionality reduction techniques, especially in large-scale graphs with nearly $10k$ node features \cite{physics_computers}. 

\noindent\textbf{Model inspection.} Authors in \cite{graph_backdoor} extend NeuralCleanse \cite{neural_cleanse} into the graph domain, which computes graph edit distance between triggers and to-be-replaced subgraphs. Krait, however, eliminates the necessity for subgraph replacement, thus restricting the effectiveness of backdoor detection. Even with the allowance for subgraph replacement, model inspection approaches will attempt to search a specific trigger in every subgraph and implement for $|\mathcal{V}|$ times, which is impractical for large-scale graphs.


\noindent\textbf{Randomized smoothing.} Randomized smoothing\cite{random_backdoor} is another potential defense mechanism, which samples numerous subgraphs of each ego-network to conduct a majority voting. Nevertheless, defending against graph prompt backdoors is impractical because the sampling operation itself has a complexity of $\mathcal{O}(|\mathcal{V}|\cdot \mathcal{C}_{s})$, where $\mathcal{C}_{s}$ is the original complexity of sampling methods. Not to mention the even more time-intensive training for all sampled subgraphs. The total computational costs are prohibitive.


\noindent\textbf{Noise filtering and injection.} Another line of defenders manipulates noises to fight against adversarial perturbations. Entezari et al. \cite{GNNSVD} empirically demonstrate that graph adversarial attacks inject noises into higher ranks in the singular value spectrum. Inspired by this phenomenon, they design GNN-SVD, which employs a low-rank approximation of the adjacency matrix to filter out high-rank noises and reset the remaining values to $1$, thus completing the pruning of noisy edges. Inversely, NoisyGNN \cite{NoisyGNN} injects noises from a pre-defined distribution into the node feature/structural space to defend against feature/structural-based adversarial attacks. To align with Krait, we implement GNN-SVD and NoisyGNN for each subgraph. We follow GNN-SVD's rank recommendation to set rank as $10$. As for NoisyGNN, we sample noises from the same Gaussian distribution $\mathcal{N}(0, \mathcal{I})$ with the default scaling parameter as $0.1$. We first inject noises into the feature spaces of the prompted subgraphs (marked as NoisyGNN-Fea) as node features play vital roles in graph prompt tuning. Next, since NoisyGNN is designed for node classification tasks and cannot be trivially adapted to graph prompt tuning which involves node-subgraph transformations, we consider a new variant of NoisyGNN (NoisyGNN-Emb) to inject noises into the graph embeddings of the prompted subgraphs. The defense performance is shown in Table \ref{krait_defense}.

% %================
\subsubsection{\textbf{Suggestions for Graph Prompt Protection}}

% Research, such as \cite{pre_conf_defense}, indicates that backdoor attacks often yield poisoned samples with statistically higher confidence scores while maintaining a relatively low PR to achieve a high ASR. Although \cite{pre_conf_defense} focuses on computer vision applications, we observe similar trends in our graph prompt tuning context as shown in Tables \ref{Krait_perf}-\ref{black_Krait}. Additionally, the poisoned candidates typically exhibit larger average degrees compared to clean samples.
% These observations suggest that monitoring nodes with unusually high prediction confidence scores and larger degrees could be an effective strategy for identifying potential threats. However, studies in fair graph learning indicate that nodes with larger degrees often play crucial roles during message-passing processes, resulting in higher confidence scores\cite{degree_bias,degree_fairness}. This implies that filtering out such nodes based solely on these criteria could significantly impair the performance of graph prompt tuning systems.
% Figure \ref{conf_score_dist} supports this, showing that the majority of both clean and poisoned samples tend to have confidence scores close to 1. Therefore, while it is valuable to be vigilant of nodes with high confidence scores, any defensive action must be carefully balanced to avoid degrading the overall system performance. This calls for a nuanced approach in monitoring and potentially flagging suspicious nodes without indiscriminately removing them, thereby preserving the integrity and effectiveness of the graph prompt tuning process.

%========================
% \subsubsection{\textbf{Suggestions for graph prompt protection}}

Wang et al. \cite{pre_conf_defense} indicate that backdoor attacks often yield statistically higher confidence scores of poisoned samples to achieve high ASRs while maintaining relatively low PRs. Although \cite{pre_conf_defense} focuses on backdoor attacks in CV, we observe similar patterns of Krait as shown in Table \ref{Krait_perf}-\ref{black_Krait}. Additionally, the poisoned candidates typically exhibit larger average degrees compared to the clean samples. The aforementioned evidence and observations inspire us to closely monitor suspicious nodes with unusually higher prediction confidence scores and larger degrees. However, previous studies in fair graph learning suggest that nodes with larger degrees enjoy more benefits during message-passing processes, resulting in higher confidence scores \cite{degree_bias,degree_fairness}. Therefore, filtering such suspicious nodes based solely on the above criteria could significantly impair the performance of graph prompt tuning. The same conclusion can be inferred from Figure \ref{conf_score_dist}, where the overwhelming majority of clean samples, as well as the poisoned samples, have confidence scores closer to $1$. Nevertheless, it is still valuable to monitor nodes with high confidence scores. 

%===================

\begin{figure}[ht]
  \centering
  \includegraphics[width=\linewidth]{conf_score.png}
  % \captionsetup{justification=raggedright,singlelinecheck=false}
  \vspace{-5mm}
  \caption{Confidence score distributions of clean and poisoned samples under three trigger generation methods.}
  \label{conf_score_dist}
  \vspace{-4mm}
\end{figure}

Another possible direction is to project suspiciously backdoored embeddings into lower dimensions to identify potential anomalies. To demonstrate whether anomalies exist under $100\%$ ASRs, we choose the ``Invoke" trigger generation method and visualize the node embeddings after one-to-one and all-to-one attacks in Figure \ref{prompt_backdoor_viz}. We observe that the poisoned samples tend to cluster at the edges of class boundaries. Therefore, comprehensively tracing nodes with high confidence scores and proximity to decision boundaries could be an effective strategy. For more detailed visualizations and analysis, please refer to Appendix \ref{Backdoored_emb_viz_appendix}. 

% Another potential strategy involves projecting suspiciously backdoored embeddings into lower dimensions to facilitate easier visualization and analysis. We demonstrate this approach with typical high-ASR attacks visualized in Figure \ref{prompt_backdoor_viz}, where it is observed that poisoned samples tend to cluster at the edges of class boundaries. This observation suggests that a comprehensive monitoring strategy that tracks nodes with both high confidence scores and proximity to decision boundaries could be effective. For more detailed visualizations and analysis, please refer to Appendix \ref{Backdoored_emb_viz_appendix}. 

\begin{figure}[H]
    \centering
    \subfloat[One-to-one attack]{  \includegraphics[width=0.4832\linewidth]{invoke_o2o_emb.png}
    \label{one-to-one}}
    \subfloat[All-to-one attack]{   \includegraphics[width=0.4832\linewidth]{invoke_a2o_emb.png}
    \label{all-to-one}}
    % \captionsetup{justification=raggedright,singlelinecheck=false}
    \vspace{-3mm}
    \caption{Backdoored node embedding of ``Invoke", poisoned nodes are marked with red circles.}
    \label{prompt_backdoor_viz}
    \vspace{-4mm}
\end{figure}
% Moreover, to prevent backdoors that utilize the 'Interact' and 'Modify' methods, defenders should either prohibit the generation of multiple graph prompts for arbitrary node sets or implement stringent scrutiny and auditing of these sets and their prompt sources to verify if they have been altered for malicious purposes. Additionally, we recommend prioritizing system-automated graph prompts over suspicious hand-crafted prompts, especially when anomalies are detected.

% \subsubsection{\textbf{Limitations and Future Work}}
% Although our empirical results showcase the effectiveness and stealthiness of Krait, we acknowledge several limitations that pave the way for future research. First, as this is the inaugural study exploring graph prompt backdoors and given the absence of a real-world Graph-Prompt-Tuning-as-a-Service (GPTaaS) environment, we are eager to test Krait under practical conditions. Second, our current methodology relies on the traditional label-flipping strategy for initializing poisoned nodes\cite{graph_backdoor, unnoticeable_graph_backdoor, explain_backdoor}; hence, adapting Krait to a clean-label scenario represents a potential direction for future development. Third, while our evaluation focuses on homophilic graphs, extending Krait's applicability to heterophilic graphs could broaden its relevance and impact. Fourth, considering that multiple graph prompts can be hand-crafted or hijacked by various attackers, this aspect of the threat model deserves further exploration. Finally, developing a more robust defense against graph prompt backdoor attacks remains a crucial objective.

%====================
Moreover, to prevent graph prompt backdoors that utilize ``Interact" and ``Modify" trigger generation methods, service providers or model/system owners should either prohibit the generation of multiple graph prompts for arbitrary node sets or implement stringent scrutiny and auditing of these sets and their prompt sources to ascertain if they have been modified for malicious purposes. Moreover, we recommend prioritizing system-automated graph prompts over potentially suspicious hand-crafted prompts, especially when anomalies are detected.

\subsubsection{\textbf{Limitations and Future Work}}
Although our empirical results showcase the attack effectiveness and stealthiness of Krait, we acknowledge several limitations that can pave the way for future work. First, despite the research surge in graph prompt tuning, there is no GPTaaS yet, we anticipate testing the performance of Krait in real-world applications. Second, we follow the classical label-flipping strategy to initialize poisoned nodes \cite{graph_backdoor, unnoticeable_graph_backdoor, explain_backdoor}, adapting Krait to the clean-label setting could be a promising direction. Third, since we only evaluate Krait in homophilic graphs, integrating Krait with heterogeneous graph prompts as triggers can further enhance its impacts. Fourth, Krait can be easily extended to multiple graph prompts, which better reflects real-world scenarios. Different attackers can handcraft or hijack different graph prompts at various times, leading to much more severe social impacts. Therefore, this problem should be further highlighted. Finally, it is critical to develop a more reliable defense mechanism against graph prompt backdoors.












%pretend as benign prompt tuning to aboveboard generate poisoned prompts as triggers and insert them to the victim ego-networks, thus precluding backdoor detection.
%, a representative to mitigate backdoors against neural networks,

% \paragraph{Logit distribution defenders} 
% One of the state-of-the-art(SOTA) backdoor defenders\cite{logit_detector} from the NLP domain employ logit distributions of the ground-truth label to detect poisoned samples in a task-agnostic way. However, AMC, which reflects the logit values of successful graph prompt backdoors, is amazingly high for almost all transfer cases, thereby impairing the defenders' capabilities. 


% Clean label.

% % Attackers as malicious outsiders distinct from users and providers. 

% Consider multiple attackers. 

% Consider directly replace prompts with triggers. 


% Identifying vunerable node candidates by exploiting non-consistent label predictions or label-non-uniformity? 



% Search for existing watermarking mechanism against backdoor attacks.
% Multi-Trigger-Key. : Toward Multi-Task Privacy Preserving in Deep Learning. IEEE ACCESS.
% Also see https://arxiv.org/abs/2210.07543.
% Also see https://proceedings.neurips.cc/paper_files/paper/2021/file/7d38b1e9bd793d3f45e0e212a729a93c-Paper.pdf backdoor unlearning and check gradients.
% Also see: https://proceedings.neurips.cc/paper_files/paper/2022/file/ec0c9ca85b4ea49c7ebfb503cf55f2ae-Paper-Conference.pdf. Comparison of Activation Values.
% Also see prediction confidence. Our key observation is that an effective black-box backdoor attack usually needs to achieve high prediction confdence on the poisoned training data, so as to ensure a high ASR. AAAI - Inspecting Prediction Confdence for Detecting Black-Box Backdoor Attacks.
% Also see proactive https://www.usenix.org/conference/usenixsecurity23/presentation/qi https://www.usenix.org/conference/usenixsecurity23/presentation/zeng : existing poisoning attacks shift data distributions, resulting in high prediction loss when training on the clean portion of a poisoned dataset and testing on the corrupted portion. 

==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

\def\mytablecaption#1{\vspace{2mm}
  \centerline{Table \arabic{mytable}.~{#1}}
  \vspace{6mm}
  \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
}


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

\def\myfigcaption#1{
             \vspace{2mm}
             \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
             \vspace{6mm}
             \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}


\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
\renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

